CARE: Lightweight Attack Resilient Secure Boot Architecturewith Onboard Recovery for RISC-V based SOC

Recent technological advancements have proliferated the use of small embedded devices for collecting, processing, and transferring the security-critical information. The Internet of Things (IoT) has enabled remote access and control of these network-connected devices. Consequently, an attacker can exploit security vulnerabilities and compromise these devices. In this context, the secure boot becomes a useful security mechanism to verify the integrity and authenticity of the software state of the devices. However, the current secure boot schemes focus on detecting the presence of potential malware on the device but not on disinfecting and restoring the soft-ware to a benign state. This manuscript presents CARE- the first secure boot framework that provides detection, resilience, and onboard recovery mechanism for the com-promised devices. The framework uses a prototype hybrid CARE: Code Authentication and Resilience Engine to verify the software state and restore it to a benign state. It uses Physical Memory Protection (PMP) and other security enchaining techniques of RISC-V processor to pro-vide resilience from modern attacks. The state-of-the-art comparison and performance analysis results indicate that the proposed secure boot framework provides a promising resilience and recovery mechanism with very little 8 % performance and resource overhead

==> relatedwork.tex <==
\section{Related work}
Existing secure boot architectures are complex \cite{UEFI:2019}, require more resources \cite{Chakraborty:2019}, \cite{Sabt:2015}, \cite{Jiang:2017}; or have been compromised by attacks such as \cite{Vasselle:2017} and \cite{Ang:2017}. SMARTS \cite{Wong:2018} uses the memory protection unit to ensure integrity. Sanctum \cite{Sanctum:2018} uses a software implementation of secure boot and crypto-core for remote attestation. The architecture proposed in \cite{Haj:2019} is a hardware root-of-trust, but it is resource-heavy as it uses a code authentication unit, a boot sequencer, a key management unit, and a TEE for secure boot. \\Other \mbox{RISC-V} based secure boot and attestation architecture such as Shakti-T \cite {Shakti:2017} uses a base and bounds concept to secure pointer access to valid memory regions. Keystone \cite{keystone} showcases a Trusted Execution Environment (TEE) with enclaves. However, none of the available solutions implements a secure boot with a recovery mechanism. Healed \cite{Healed:2019} has demonstrated the first recovery mechanism using Merkle Hash Tree (MHT), which assumes at least one node in the network is untampered, and the node's firmware can be used to reflash corrupted nodes. \\Another implementation \cite{Secerase2010} has shown a method of inserting software receiver-transmitter code into trusted ROM to associate with a recovery server. However, they do not support secure boot architecture. Our method uses a different approach to storing recovery data in secure ROM. To the best of our knowledge, ours is the first implementation of a \emph{hybrid lightweight, secure boot architecture with and an onboard resilience engine} for \mbox{RISC-V} based devices.

\par This section gives an overview of the most common techniques for secure boot and remote attestation. Remote attestation is a process of remotely verifying the state of the software running on the untrusted device.  RA measures the cryptographic digest of the software running on the untrusted device. Previous researchers have implemented RA's which can be classified in three categories namely hardware, software or hybrid. \\
{\bf{Hardware Based}:} One of the most popular method of RA uses a discrete co-processor called Trusted Platform Module (TPM) \cite{Tpm:2010} recommended by Trusted Computing Group (TCG). TPM has some special purpose registers called Platform Configuration Registers (PCRs). PCRs cannot be overwritten but can only extended by hashing of software measurements together with previous PCR values. The TPM can sign the PCRs with an private attestation key in order to generate an attestation evidence. The TPM provides hardware root-of-trust, but due to space, size, and cost constraints it is not suitable for small embedded or IoT devices.
\par Some researchers have used Trusted Execution Environment (TEE) \cite{Sabt:2015} or proprietary implementation of Arm TrustZone \cite{Jiang:2017}. TrustZone uses two virtual processors known as secure world and normal world. The isolation between them is enforced by hardware. Microsoft’s fTPM \cite{mcs:2015} provides a usecase of TrustZone for secure boot and attestation. Intel's SGX \cite{sgx:2013} provides instruction and memory access features that can be used to instantiate protected containers referred as enclaves by using special instructions and processor extensions. TrustZone and TEE increases design complexity and cost due to exclusive licensing. Some secure boot architectures uses Unified Extensible Firmware Interface (UEFI) \cite{NSA}, which is complex in design and not suitable for small embedded and IoT devices.\\
{\bf{Software Based}:} Other researchers have used simulated or software TPM implementations like simTPM \cite{Chakraborty:2019} or IBM's software TPM \cite{Goldman}. RISC-V based implementation Sanctum \cite{Sanctum:2018} uses software based secure boot for remote attestation. Another software implementation \cite{ndss:2018} uses software cryptographic core and hash engine for RA. Software root-of-trust are prone to malware attacks and considered less secure. \\
{\bf{Hybrid}:} SMART \cite{Wong:2018} is a dynamic root-of-trust architecture for low-end devices at runtime. SPM/Sancus: SPM \cite{Stra:2010} and Sancus \cite{sancus:2013} present a security architecture which provides isolation of software modules using additional CPU instructions. TrustLite/TyTAN: TrustLite \cite{TrustLite:2014} and its successor TyTAN \cite{TyTan:2015} provide flexible, hardware-enforced isolation of software modules using Execution-Aware Memory Protection Unit (EA-MPU) in hardware.

\par Some other RISC-V based secure boot and attestation architecture like Shakti-T \cite {Shakti:2017} uses base and bounds concept to secure pointer's access to valid memory regions. Keystone \cite{keystone} showcases a trusted execution environment (TEE) with enclaves. Lightweight secure boot work proposed in \cite{Haj:2019} represents a hardware based secure boot. However, it requires a lot of hardware resources like two RISC-V 64 bit processors for TEE implementation, key management unit, PUF module, additional hardware for cryptographic hashing (SHA3), and asymmetric cryptographic core  Elliptic Curve Digital Signature Algorithm-(ECDSA) for signing the software. This makes it \cite{Haj:2019} not suitable for lightweight small embedded or IoT applications. Recent opensource root-of-trust project from Google called Opentitan \cite{Ope:2019} provides sample implementation of secure boot. However, none of the available solution has secure recovery mechanism. Healed \cite{Healed:2019} has demonstrated the first recovery mechanism using Merkle Hash Tree (MHT), which assumes atleast one node in the network is untempered and firmware of it can be used to reflash corrupted nodes. Another implementation \cite{Secerase:2010} has shown a method of putting siftware receiver-transmitter code into trusted ROM for connecting to a recovery server which also requires additional ROM storage.  Proposed method uses different approach of storing recovery data in backup secure ROM for small embedded IoT application. To the best of our knowledge proposed work is the first implementation of a \emph{hardware based lightweight RA and secure boot architecture with on board resilience engine} for RISC-V based resource contrained embedded or IoT systems. 

\par Studies have shown that attacks like laser induced fault injection \cite{Vasselle:2017} and second order pulse electromagnetic fault injection \cite{Ang:2017} have compromised some of the secure boot architectures.


